Enclosed mmWave Wearable Networks: Feasibility and Performance

This paper investigates the feasibility of mmWave frequencies for personal networks of wireless wearable devices in enclosed settings (e.g., commuter trains, subways, airplanes, airports, or offices). At these frequencies, specular reflections off surfaces are expected to contribute intended signal power and, simultaneously, to aggravate the interference at the receivers. Meanwhile, blockages by obstacles and people---including the individuals wearing the devices---are expected to shield receivers from interference. With the aid of stochastic geometry and random shape theory, we assess the interplay of surface reflections and blockages for dense deployments of wearable networks equipped with directional antenna arrays in relevant indoor settings.

==> delitest.tex <==
% Copyright 2007 TeX Users Group.
% You may freely use, modify and/or distribute this file.
\typesize=10pt

\input lcdplain.mac

% For CM:

% \def\big#1{{\hbox{$\left#1\vbox to8.5\p@{}\right.\n@space$}}}
% \def\Big#1{{\hbox{$\left#1\vbox to11.5\p@{}\right.\n@space$}}}
% \def\bigg#1{{\hbox{$\left#1\vbox to14.5\p@{}\right.\n@space$}}}
% \def\Bigg#1{{\hbox{$\left#1\vbox to17.5\p@{}\right.\n@space$}}}

% Even bigger sizes than plain provides.
\def\biggg#1{{\hbox{$\left#1\vbox to20.5pt{}\right.$}}}
\def\bigggl{\mathopen\biggg}
\def\bigggr{\mathclose\biggg}
\def\Biggg#1{{\hbox{$\left#1\vbox to23.5pt{}\right.$}}}
\def\Bigggl{\mathopen\Biggg}
\def\Bigggr{\mathclose\Biggg}

% for LucidaNewMath:

% \def\big#1{{\hbox{$\left#1\vbox to8.63\p@{}\right.\n@space$}}}
% \def\Big#1{{\hbox{$\left#1\vbox to11.37\p@{}\right.\n@space$}}}
% \def\bigg#1{{\hbox{$\left#1\vbox to14.13\p@{}\right.\n@space$}}}
% \def\Bigg#1{{\hbox{$\left#1\vbox to16.87\p@{}\right.\n@space$}}}

% Even bigger sizes than plain provides.
\def\biggg#1{{\hbox{$\left#1\vbox to19.62pt{}\right.$}}}
\def\bigggl{\mathopen\biggg}
\def\bigggr{\mathclose\biggg}
\def\Biggg#1{{\hbox{$\left#1\vbox to22.37pt{}\right.$}}}
\def\Bigggl{\mathopen\Biggg}
\def\Bigggr{\mathclose\Biggg}

$$
\Bigggl(\bigggl(\Biggl(\biggl(\Bigl(\bigl(({x})\bigr)\Bigr)\biggr)\Biggr)\bigggr)\Bigggr)
% $$
\quad 
% $$
\Bigggl[\bigggl[\Biggl[\biggl[\Bigl[\bigl[[{x}]\bigr]\Bigr]\biggr]\Biggr]\bigggr]\Bigggr]
% $$
% $$
% \Bigggl\lbrack\bigggl\lbrack\Biggl\lbrack\biggl\lbrack\Bigl\lbrack\bigl\lbrack\lbrack{x}\rbrack\bigr\rbrack\Bigr\rbrack\biggr\rbrack\Biggr\rbrack\bigggr\rbrack\Bigggr\rbrack
% $$
\quad  
% $$
\Bigggl\{\bigggl\{\Biggl\{\biggl\{\Bigl\{\bigl\{\{{x}\}\bigr\}\Bigr\}\biggr\}\Biggr\}\bigggr\}\Bigggr\}
$$
% $$
% \Bigggl\lbrace\bigggl\lbrace\Biggl\lbrace\biggl\lbrace\Bigl\lbrace\bigl\lbrace\lbrace{x}\rbrace\bigr\rbrace\Bigr\rbrace\biggr\rbrace\Biggr\rbrace\bigggr\rbrace\Bigggr\rbrace
% $$

$$
\Bigggl\lmoustache\bigggl\lmoustache\Biggl\lmoustache\biggl\lmoustache\Bigl\lmoustache\bigl\lmoustache\lmoustache{x}\rmoustache\bigr\rmoustache\Bigr\rmoustache\biggr\rmoustache\Biggr\rmoustache\bigggr\rmoustache\Bigggr\rmoustache
% $$
\quad  
% $$
\Bigggl\lceil\bigggl\lceil\Biggl\lceil\biggl\lceil\Bigl\lceil\bigl\lceil\lceil{x}\rceil\bigr\rceil\Bigr\rceil\biggr\rceil\Biggr\rceil\bigggr\rceil\Bigggr\rceil
% $$
\quad  
% $$
\Bigggl\lfloor\bigggl\lfloor\Biggl\lfloor\biggl\lfloor\Bigl\lfloor\bigl\lfloor\lfloor{x}\rfloor\bigr\rfloor\Bigr\rfloor\biggr\rfloor\Biggr\rfloor\bigggr\rfloor\Bigggr\rfloor
$$

$$
\Bigggl\langle\bigggl\langle\Biggl\langle\biggl\langle\Bigl\langle\bigl\langle\langle{x}\rangle\bigr\rangle\Bigr\rangle\biggr\rangle\Biggr\rangle\bigggr\rangle\Bigggr\rangle
% $$
\quad  
% $$
\Bigggl\backslash\bigggl\backslash\Biggl\backslash\biggl\backslash\Bigl\backslash\bigl\backslash\backslash{x}/\bigr/\Bigr/\biggr/\Biggr/\bigggr/\Bigggr/
$$

$$
\Bigggl\lgroup\bigggl\lgroup\Biggl\lgroup\biggl\lgroup\Bigl\lgroup\bigl\lgroup\lgroup{x}\rgroup\bigr\rgroup\Bigr\rgroup\biggr\rgroup\Biggr\rgroup\bigggr\rgroup\Bigggr\rgroup
% $$
\quad  
% $$
\Bigggl\uparrow\bigggl\uparrow\Biggl\uparrow\biggl\uparrow\Bigl\uparrow\bigl\uparrow\uparrow{x}\downarrow\bigr\downarrow\Bigr\downarrow\biggr\downarrow\Biggr\downarrow\bigggr\downarrow\Bigggr\downarrow
$$

$$
\Bigggl\Uparrow\bigggl\Uparrow\Biggl\Uparrow\biggl\Uparrow\Bigl\Uparrow\bigl\Uparrow\Uparrow{x}\Downarrow\bigr\Downarrow\Bigr\Downarrow\biggr\Downarrow\Biggr\Downarrow\bigggr\Downarrow\Bigggr\Downarrow
% $$
\quad  
% $$
\Bigggl\updownarrow\bigggl\updownarrow\Biggl\updownarrow\biggl\updownarrow\Bigl\updownarrow\bigl\updownarrow\updownarrow{x}\Updownarrow\bigr\Updownarrow\Bigr\Updownarrow\biggr\Updownarrow\Biggr\Updownarrow\bigggr\Updownarrow\Bigggr\Updownarrow
$$

$$
\Bigggl\arrowvert\bigggl\arrowvert\Biggl\arrowvert\biggl\arrowvert\Bigl\arrowvert\bigl\arrowvert\arrowvert{x}\Arrowvert\bigr\Arrowvert\Bigr\Arrowvert\biggr\Arrowvert\Biggr\Arrowvert\bigggr\Arrowvert\Bigggr\Arrowvert
% $$
\quad
% $$
\Bigggl\Vert\bigggl\Vert\Biggl\Vert\biggl\Vert\Bigl\Vert\bigl\Vert\Vert{x}\vert\bigr\vert\Bigr\vert\biggr\vert\Biggr\vert\bigggr\vert\Bigggr\vert
% $$
\quad
% $$
\Bigggl\bracevert\bigggl\bracevert\Biggl\bracevert\biggl\bracevert\Bigl\bracevert\bigl\bracevert\bracevert{x}\bracevert\bigr\bracevert\Bigr\bracevert\biggr\bracevert\Biggr\bracevert\bigggr\bracevert\Bigggr\bracevert
$$

\end

